Modeling Temporal Data as Continuous Functions with Stochastic Process Diffusion

Temporal data such as time series can be viewed as discretized measurements of the underlying function. To build a generative model for such data we have to model the stochastic process that governs it. We propose a solution by defining the denoising diffusion model in the function space which also allows us to naturally handle irregularly-sampled observations. The forward process gradually adds noise to functions, preserving their continuity, while the learned reverse process removes the noise and returns functions as new samples. To this end, we define suitable noise sources and introduce novel denoising and score-matching models. We show how our method can be used for multivariate probabilistic forecasting and imputation, and how our model can be interpreted as a neural process.

==> sections/continuous.tex <==
\section{Continuous diffusion}\label{sec:continuous_diffusion}

\subsection{Background: Score-based SDEs}

Instead of taking a finite number of diffusion steps as in \Secref{sec:discrete}, we can introduce a continuous diffusion $\vx_0 \mapsto \vx_\diffusionContInd$ where $\diffusionContInd \in [0, \diffusionContLast]$ is a continuous variable. The diffusion can be modeled with a stochastic differential equation \citep{song2021sde}:
\begin{align}\label{eq:diffusion_sde}
    \diff \vx_\diffusionContInd = f(\vx_\diffusionContInd, \diffusionContInd) \diff \diffusionContInd + g(\diffusionContInd) \diff W_\diffusionContInd,
\end{align}
where $W$ is a Wiener process. The variable $\diffusionContInd$ is the diffusion time so the input gets noisier as more time passes. This should not be confused with the time of our time series $t$.
For a forward SDE (\Eqref{eq:diffusion_sde}) there exist the corresponding reverse SDE, solved from $\diffusionContLast$ to $0$:
\begin{align}\label{eq:reverse_sde}
    \diff \vx_\diffusionContInd = [f(\vx_\diffusionContInd, \diffusionContInd) - g(\diffusionContInd)^2 \score] \diff \diffusionContInd + g(\diffusionContInd) \diff W_\diffusionContInd .
\end{align}
%
The generative model learns the so-called score function $\score$ with a neural network $\scoreNet(\vx_\diffusionContInd, \diffusionContInd)$. The loss is then \citep{song2021sde}:
\begin{align}
    \mathcal{L}(\vx_0) = \E_{\diffusionContInd \sim \mathcal{U}(0, \diffusionContLast)}
    \left[|| 
        \scoreNet(\vx_\diffusionContInd, \diffusionContInd) - \score
    ||_2^2 \right] .
\end{align}
The sampling can then be performed by first sampling the initial value $\vx_\diffusionContLast \sim p(\vx_\diffusionContLast)$ (depends on \Eqref{eq:diffusion_sde}) and then solving \Eqref{eq:reverse_sde} or the probability flow as described in \citet{song2021sde}.



==> sections/discrete.tex <==
\section{Discrete diffusion}\label{sec:discrete}

\subsection{Background: DDPM}

\citet{ho2020denoising} propose a denoising diffusion probabilistic model (DDPM) where they gradually add noise to the observed data point $\vx_0$, essentially defining a sequence of progressively noisier values $\vx_1, \vx_2, \dots, \vx_\diffusionLast$. The final value $\vx_\diffusionLast \sim \mathcal{N}(\vzero, \vone)$ carries no information about the original data point. The goal is to learn to reverse this process.

The diffusion forms a Markov chain where the transition between any two consecutive points is defined with a conditional probability $q(\vx_\diffusionInd | \vx_{\diffusionInd-1}) = \mathcal{N}(\sqrt{1-\beta_\diffusionInd} \vx_{\diffusionInd-1}, \beta_\diffusionInd \mI)$. The sequence of noise scales $\beta_1, \dots, \beta_\diffusionLast$ is increasing such that the first noisy value $\vx_1$ is close to the data $\vx_0$, and the final value $\vx_\diffusionLast$ is pure noise.

For convenience, we define $\alpha_\diffusionInd = 1 - \beta_\diffusionInd$ and $\bar{\alpha}_\diffusionInd = \prod_{k=1}^\diffusionInd \alpha_k$. Since our transition kernel is a normal distribution, the value at any step $\diffusionInd$ can be calculated directly from the given data point $\vx_0$:
\begin{align}\label{eq:q_xi_x0}
    q(\vx_\diffusionInd | \vx_0) = \mathcal{N}(\sqrt{\bar{\alpha}_\diffusionInd} \vx_0, (1 - \bar{\alpha}_\diffusionInd) \mI).
\end{align}
Sampling $\vx_\diffusionInd$ conditioned on $\vx_0$ is straightforward:
\begin{align}\label{eq:ddpm_sample_xn}
    \vx_\diffusionInd = \sqrt{\bar\alpha_\diffusionInd} \vx_0 + \sqrt{1 - \bar\alpha_\diffusionInd} \noise, \quad \noise \sim \mathcal{N}(\vzero, \mI).
\end{align}
Further, we can derive the probability of any intermediate value $\vx_{\diffusionInd-1}$ given its successor $\vx_\diffusionInd$ as:
\begin{align}\label{eq:q_posterior}
    &q(\vx_{\diffusionInd-1} | \vx_\diffusionInd, \vx_0) = \mathcal{N}(\tilde{\vmu}_\diffusionInd, \tilde\beta_\diffusionInd \mI),\\
\text{where:}\quad
    &\tilde{\vmu}_\diffusionInd = \frac{\sqrt{\bar{\alpha}_{\diffusionInd-1}} \beta_\diffusionInd}{1 - \bar{\alpha}_\diffusionInd} \vx_0 + \frac{\sqrt{\alpha_\diffusionInd} (1 - \bar\alpha_{\diffusionInd-1})}{1 - \bar\alpha_\diffusionInd} \vx_\diffusionInd, \qquad 
    \tilde\beta_\diffusionInd = \frac{1 - \bar{\alpha}_{\diffusionInd-1}}{1 - \bar{\alpha}_\diffusionInd} \beta_\diffusionInd .
\end{align}
%
The generative model is the reverse process $p(\vx_{\diffusionInd-1} | \vx_\diffusionInd)$ that we have to learn. To sample a new point, we start at $\vx_\diffusionLast \sim \mathcal{N}(\vzero, \vone)$ and iteratively denoise it ($\vx_\diffusionLast \mapsto \vx_{\diffusionLast -1} \mapsto \dots \mapsto \vx_0$) until we get a sample from the data distribution.

\citet{ho2020denoising} set $p(\vx_{i-\diffusionInd} | \vx_\diffusionInd) = \mathcal{N}(\vmu_\theta(\vx_\diffusionInd, i), \beta_\diffusionInd \mI)$, where $\vmu_\theta$ is parameterized by a neural network. To train the model they optimize the loss --- the KL-divergence between the known distribution $q(\vx_{\diffusionInd-1} | \vx_\diffusionInd, \vx_0)$ and the learned distribution $p(\vx_{\diffusionInd-1} | \vx_\diffusionInd)$. Since all distributions are normal, this can be simplified to the following loss:
\begin{align}\label{eq:loss_ddpm}
    \mathcal{L}(\vx_0) = \E_{\noise \sim \mathcal{N}(\vzero, \mI),\diffusionInd \sim \mathcal{U}(0, \diffusionLast)}\left[|| \vmu_\theta(\vx_\diffusionInd, \diffusionInd) - \noise ||_2^2\right].
\end{align}
In summary, the forward process adds the noise $\noise$ at different scales to the input $\vx_0$ to produce $\vx_\diffusionInd$ while the model learns to invert this, i.e., predicts the noise $\noise$ from $\vx_\diffusionInd$.


\subsection{Our model}

We consider a time series $(\vx_{0}(t_1), \dots, \vx_{0}(t_\timeSeriesSize))$ consisting of $\timeSeriesSize$ points observed at times $\mathcal{T} = \{ t_1, \dots, t_\timeSeriesSize \}$. The times $t \in \mathcal{T}$ can be equally spaced as is the case in the traditional time series datasets, but this formulation also encompasses the irregularly-sampled data when $t \in \mathcal{T} \subset \R_{+}$. 

We assume the values $\vx_{0}(t)$ follow some continuous function in time $f : \mathcal{T} \to \R^d$. For example, the temperature measurements are a set of discrete observations but there is always \emph{some} temperature value, even when we are not measuring it, and its function of time is smooth.

We want to design a generative model that produces samples $\vx_0(t)$. The samples can be viewed as functions that take time as input and output data points corresponding to a time series. If we try to apply the DDPM approach to this setting directly, the resulting sample will almost surely be discontinuous since the noising process adds independent noise to every pair of distinct time points. In the following, we present the alternative that adds noise coming from a stochastic process.

As data $\{\vx_{0}(t)\}_{t \in \mathcal{T}}$ follows some underlying function $f$, we are interested in modeling ``$p(f)$", i.e., we want to capture the stochastic process. Instead of viewing the diffusion as adding noise to a vector, we add noise to the whole function at once, thus, the noise has to be a function as well. For every time point $t$, we write the diffused value after $\diffusionInd$ steps as
\begin{align}
    \vx_\diffusionInd(t) = \sqrt{\bar\alpha_\diffusionInd} \vx_0(t) + \sqrt{1 - \bar\alpha_\diffusionInd} \noise(t),
\end{align}
where $\vx_0(t)$ is the given time series data point and $\vx_\diffusionInd(t)$ is the noisy output produced by adding time dependent noise $\noise(t)$. If $\vx_0(t)$ and $\noise(t)$ are continuous functions then $\vx_\diffusionInd(t)$ will be continuous. Further, we would like to converge to some known process after $\diffusionLast$ diffusion steps.

Consider obtaining the noise from a standard Wiener process (Brownian motion) $\noise(t) = W(t)$. A clear disadvantage of this approach is that variance grows with time. Additionally, at $t=0$ we never add any noise which can be solved in an ad hoc manner by shifting the whole time series similar to \citet{deng2020modeling}. Instead, in the following, we present two stationary stochastic processes that add the same amount of noise irrespective of time $t$ and reduce to DDPM in the trivial case when our time series has only one element.

\textbf{Gaussian process diffusion.} Given a set of points $\mathcal{T}$, we propose sampling $\{ \noise(t) \}_{t \in \mathcal{T}}$ from a Gaussian process $\mathcal{N}(\vzero, \mSigma)$, where each element of the covariance matrix is specified with a kernel $\mSigma_{s,t} = k(s, t)$, e.g., with a radial basis function. This produces \emph{smooth} noise samples $\noise(t)$ and the final result of diffusion after $N$ steps $\{\vx_\diffusionLast(t)\}_{t\in \mathcal{T}}$ follows the same Gaussian process $\mathcal{N}(\vzero, \mSigma)$.

\textbf{Ornstein-Uhlenbeck diffusion.} The alternative noise distribution is a stationary OU process which is specified as a solution to the following stochastic differential equation:
\begin{align}\label{eq:ou_sde}
    d\noise(t) = -\alpha \noise(t) dt + dW(t),
\end{align}
where $W(t)$ is the standard Wiener process and we use the initial condition $\noise(0) \sim \mathcal{N}(0, 1)$. We can obtain samples from OU process easily by sampling from a modified Wiener process: $e^{-\alpha t} W(e^{2 \alpha  t})$. The covariance can be calculated as $\mathrm{cov}(s, t) = e^{-\alpha |s - t|}$.
The OU process is a special case of a Gaussian process when using Mat\'ern kernel with $\nu = 0.5$ \cite[p.\ 86]{williams2006gaussian}.

\textbf{Diffusion.} 
Given a finite number of data points $\{\vx_{0}(t)\}_{t \in \mathcal{T}}$, we calculate the sample from a stochastic process $\noise(t)$ at points $t \in \mathcal{T}$ by sampling from a multivariate normal distribution $\mathcal{N}(\vzero, \mSigma)$ in case we use Gaussian process diffusion or from a modified Wiener process for OU diffusion. Following the convention from DDPM, the transition kernel is
\begin{align}
    q(\vx_\diffusionInd | \vx_0) = \mathcal{N}(\sqrt{\bar{\alpha}_\diffusionInd} \vx_0, (1 - \bar{\alpha}_\diffusionInd) \mSigma),
\end{align}
and the posterior can be written as:
\begin{align}
    q(\vx_{\diffusionInd-1} | \vx_\diffusionInd, \vx_0) = \mathcal{N}(\tilde{\vmu}_\diffusionInd, \tilde\beta_\diffusionInd \mSigma),
\end{align}
where $\tilde{\vmu}_\diffusionInd$ and $\tilde\beta_\diffusionInd$ are calculated the same way as in \Eqref{eq:q_posterior}, see \Appref{app:ddpm_posterior} for full derivation.

\textbf{The loss} is again the KL divergence which, as it turns out, can be written in the same form as in \Eqref{eq:loss_ddpm} (see \Appref{app:ddpm_loss}). The difference is that instead of single data points, we now have a set of observations and want to predict a set of noise values $\smash{\noise \in \R^{\timeSeriesSize \times d}}$:
\begin{align}\label{eq:ddpm_continuous_loss}
    \mathcal{L}(\{ \vx_0(t) \}_{t\in\mathcal{T}}) = \E_{\noise \sim \mathcal{N}(\vzero, \mI),\diffusionInd \sim \mathcal{U}(0, \diffusionLast)}\left[|| 
    \noise - \noise_\theta(\{ (\vx_\diffusionInd(t), t) \}_{t\in\mathcal{T}}, \diffusionInd) ||_2^2\right].
\end{align}


\textbf{Sampling} from our generative model is similar to the algorithm from \citet{ho2020denoising} but the noise comes from a Gaussian or OU process (Algorithm~\ref{alg:sampling_ddpm}), instead of using independent white noise.


\begin{minipage}{0.44\textwidth}
    \begin{algorithm}[H]
    \centering
    \caption{Training with OU diffusion}\label{alg:training_ddpm}
    \footnotesize
    \begin{algorithmic}[1]
        \Repeat
        \State $\{ (\vx_0(t), t) \} \sim p_\text{data}$
        \State $\mSigma_{u, v} = \exp(-\alpha |u - v|)$
        \State $\noise \sim \mathcal{N}(\vzero, \mSigma)$
        \State $\diffusionInd \sim \mathcal{U}(1, \diffusionLast)$
        \State Take gradient step on
        \State \indent $\nabla_\theta || \noise - \noise_\theta(\{ (\vx_\diffusionInd(t), t) \}, \diffusionInd) ||_2^2$
        \Until{converged}
    \end{algorithmic}
    \end{algorithm}
\end{minipage}
\begin{minipage}{0.55\textwidth}
    \begin{algorithm}[H]
    \centering
    \caption{Sampling with OU diffusion}\label{alg:sampling_ddpm}
    \footnotesize
    \begin{algorithmic}[1]
        \State \textbf{input:} $\{ t_1, \dots, t_\timeSeriesSize \}$
        \For{$\diffusionInd = \diffusionLast, \dots, 1$}
            \State $\vz(t) \sim e^{-\alpha t} W(e^{2 \alpha t})$
            \State $\vx_{\diffusionInd - 1}(t) = \frac{1}{\sqrt{\alpha_\diffusionInd}} \left( \vx_\diffusionInd(t) - \frac{1 - \alpha_\diffusionInd}{\sqrt{1 - \bar\alpha_\diffusionInd}}
            \noise_\theta(t)
            \right) + \sigma_\diffusionInd \vz$
        \EndFor
        \State \textbf{return} $\{ \vx_0(t) \}$
    \end{algorithmic}
    \end{algorithm}
\end{minipage}

